Look Ma, no markers: holistic performance capture without the hassle

We tackle the problem of highly-accurate, holistic performance capture for the face, body and hands simultaneously. Motion-capture technologies used in film and game production typically focus only on face, body or hand capture independently, involve complex and expensive hardware and a high degree of manual intervention from skilled operators. While machine-learning-based approaches exist to overcome these problems, they usually only support a single camera, often operate on a single part of the body, do not produce precise world-space results, and rarely generalize outside specific contexts. In this work, we introduce the first technique for marker-free, high-quality reconstruction of the complete human body, including eyes and tongue, without requiring any calibration, manual intervention or custom hardware. Our approach produces stable world-space results from arbitrary camera rigs as well as supporting varied capture environments and clothing. We achieve this through a hybrid approach that leverages machine learning models trained exclusively on synthetic data and powerful parametric models of human shape and motion. We evaluate our method on a number of body, face and hand reconstruction benchmarks and demonstrate state-of-the-art results that generalize on diverse datasets.

==> figures/face_model_comp.tex <==
\begin{figure}
    \centering
    \footnotesize
    \includegraphics[width=.496\linewidth]{figures/moai_comp/1.jpg}
    \hfill
    \includegraphics[width=.496\linewidth]{figures/moai_comp/5.jpg}
    % \includegraphics[width=.496\linewidth]{figures/moai_comp/3.jpg}
    % \hfill
    % \includegraphics[width=.496\linewidth]{figures/moai_comp/6.jpg}\\
    \caption{Comparison of retoplogized training scan (left) to fits using face model of \citet{wood2021fake} (middle) and our face model (right). Significantly more high frequency detail is captured and lip definition is improved.}
    \label{fig:face_model_comp}
\end{figure}
